Approximation of nearly-periodic symplectic maps via structure-preserving neural networks

A continuous-time dynamical system with parameter $\varepsilon$ is nearly-periodic if all its trajectories are periodic with nowhere-vanishing angular frequency as $\varepsilon$ approaches 0. Nearly-periodic maps are discrete-time analogues of nearly-periodic systems, defined as parameter-dependent diffeomorphisms that limit to rotations along a circle action, and they admit formal $U(1)$ symmetries to all orders when the limiting rotation is non-resonant. For Hamiltonian nearly-periodic maps on exact presymplectic manifolds, the formal $U(1)$ symmetry gives rise to a discrete-time adiabatic invariant. In this paper, we construct a novel structure-preserving neural network to approximate nearly-periodic symplectic maps. This neural network architecture, which we call symplectic gyroceptron, ensures that the resulting surrogate map is nearly-periodic and symplectic, and that it gives rise to a discrete-time adiabatic invariant and a long-time stability. This new structure-preserving neural network provides a promising architecture for surrogate modeling of non-dissipative dynamical systems that automatically steps over short timescales without introducing spurious instabilities.

==> NPMap arXiv/figure4.tex <==
{
\newcommand{\figWidth}{8.5cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.0}{.0}{.0}{.0}}
\begin{figure}[!htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.,.7) rectangle (16,17.5);  % set the bounding box (so we have less surrounding white space)
\draw(-1.18,0) node[anchor=south west] {\trimfig{eps_0.11_Oscillator1}{\figWidth}};
\draw(7.59,0) node[anchor=south west] {\trimfig{eps_0.11_Oscillator2}{\figWidth}};
\node at (7.08,.6) {\small$(q_1, p_1)$};
\node at (15.83,.6) {\small$(q_2, p_2)$};
%
\begin{scope}[yshift=4.55cm]
\draw(-1.18,0) node[anchor=south west] {\trimfig{eps_0.07_Oscillator1}{\figWidth}};
\draw(7.59,0) node[anchor=south west] {\trimfig{eps_0.07_Oscillator2}{\figWidth}};
\node at (7.08,.6) {\small$(q_1, p_1)$};
\node at (15.83,.6) {\small$(q_2, p_2)$};
\end{scope}
%
\begin{scope}[yshift=9.1cm]
\draw(-1.18,0) node[anchor=south west] {\trimfig{eps_0.02_Oscillator1}{\figWidth}};
\draw(7.59,0) node[anchor=south west] {\trimfig{eps_0.02_Oscillator2}{\figWidth}};
\node at (7.06,.6) {\small$(q_1, p_1)$};
\node at (15.83,.6) {\small$(q_2, p_2)$};
\end{scope}
%
\begin{scope}[yshift=13.65cm]
\draw(-1.18,0) node[anchor=south west] {\trimfig{eps_0_Oscillator1}{\figWidth}};
\draw(7.59,0) node[anchor=south west] {\trimfig{eps_0_Oscillator2}{\figWidth}};
\node at (7.08,.6) {\small$(q_1, p_1)$};
\node at (15.83,.6) {\small$(q_2, p_2)$};
\end{scope}
% background grid:
%\draw[step=1cm,gray] (0,0) grid (16,17.5);
\end{tikzpicture}
\end{center}
\vspace{2mm}
\caption{Sample trajectories in $(q_1,p_1)$ and $(q_2,p_2)$ phase spaces (left column: first oscillator, right column: second oscillator) for the nearly-periodic Hamiltonian system~\eqref{eq: Example of Interest Equations} as the value of the parameter $\varepsilon$ is increased.\label{fig: Trajectories}}
\end{figure}
}

==> NPMap arXiv/figure5.tex <==
{
\newcommand{\figWidth}{8.6cm}
\newcommand{\figWidthb}{8.5cm}
\newcommand{\figWidthc}{9.5cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.0}{.0}{.0}{.0}}
\begin{figure}[!ht]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.,.7) rectangle (16,9.7);  % set the bounding box (so we have less surrounding white space)
\draw(-1.2,0) node[anchor=south west] {\trimfig{Reference_Oscillator2}{\figWidthb}};
\draw(7.7,0) node[anchor=south west] {\trimfig{NN_Model_Prediction_Oscillator2}{\figWidth}};
\node at (7.1,.6) {\small$(q_2, p_2)$};
\node at (16.1,.6) {\small$(q_2, p_2)$};
%
\draw(2.8,4.6) node[anchor=south west] {\trimfig{Level_Sets}{\figWidthc}};
\node at (12.,5.2) {\small$(q_2, p_2)$};
% background grid:
% \draw[step=1cm,gray] (0,0) grid (16,9.7);
\end{tikzpicture}
\end{center}
\caption{Level sets of the averaged Hamiltonian~\eqref{eq: approximate averaged Hamiltonian}, and the symplectic gyroceptron predictions against the reference trajectories for the second oscillator in the nearly-periodic Hamiltonian system~\eqref{eq: Example of Interest Equations} with $\varepsilon = 0.01$ and a time-step of 0.05.\label{fig: Learnt Dynamics}}
\end{figure}
\vspace{-2mm}
}


==> NPMap arXiv/figure6.tex <==
{
\newcommand{\figWidth}{8.7cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.0}{.0}{.0}{.0}}
\begin{figure}[!ht]
	\vspace{-2mm}
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.,.7) rectangle (16,9.7);  % set the bounding box (so we have less surrounding white space)
\draw(-1.2,0) node[anchor=south west] {\trimfig{LargeOscillator_SympNet}{\figWidth}};
\draw(7.65,0) node[anchor=south west] {\trimfig{LargeOscillator_HenonNet}{\figWidth}};
\node at (7.3,.6) {\small$(q_2, p_2)$};
\node at (16.2,.6) {\small$(q_2, p_2)$};
%
\begin{scope}[yshift=4.8cm]
\draw(-1.2,0) node[anchor=south west] {\trimfig{LargeOscillator_Reference}{\figWidth}};
\draw(7.65,0) node[anchor=south west] {\trimfig{LargeOscillator_SymplecticGyroceptron}{\figWidth}};
\node at (7.3,.6) {\small$(q_2, p_2)$};
\node at (16.2,.6) {\small$(q_2, p_2)$};
\end{scope}
% background grid:
% \draw[step=1cm,gray] (0,0) grid (16,9.7);
\end{tikzpicture}
\end{center}\caption{Predictions from a Symplectic Gyroceptron, a SympNet, and a HenonNet, against the reference trajectories for the second oscillator in the nearly-periodic Hamiltonian system~\eqref{eq: Example of Interest Equations} with $\varepsilon = 0.01$ and the larger time-step of 5. \label{fig: Learnt Dynamics_BigStep}} \vspace{-3.5mm}
\end{figure}
}

==> NPMap arXiv/figure_adiabatic.tex <==
{
\newcommand{\figWidth}{4.6cm}
\newcommand{\trimfig}[2]{\trimh{#1}{#2}{.0}{.0}{.0}{.0}}
\begin{figure}[!ht]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.4,1.2) rectangle (13,5.3);  % set the bounding box (so we have less surrounding white space)
  \draw(0,.5) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{Adiabatic}{\figWidth}};
 \node at (12.3,0.7) {\small$\epsilon$};
 \node at (.35,5.15) {\small$N(\epsilon)$};
% background grid:
% \draw[step=1cm,gray] (0,0) grid (13,5.3);
\end{tikzpicture}
\end{center}
\caption{ $N(\varepsilon)$ as a function of $\varepsilon$ for $\rho = 1.1$ and a random set of weights. \label{fig: Adiabatic} }
\end{figure}
}

==> NPMap arXiv/figure_iteration.tex <==
{
\newcommand{\figWidth}{8.5cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.0}{.0}{.0}{.0}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.,.7) rectangle (16,12.1);  % set the bounding box (so we have less surrounding white space)
\draw(-1.,0) node[anchor=south west] {\trimfig{Profile_eps5}{\figWidth}};
\draw(7.7,0) node[anchor=south west] {\trimfig{Profile_eps1}{\figWidth}};
\node at (-.7,1.6) {\small$\mu$};
%
\begin{scope}[yshift=3cm]
\draw(-1.,0) node[anchor=south west] {\trimfig{Profile_eps6}{\figWidth}};
\draw(7.7,0) node[anchor=south west] {\trimfig{Profile_eps2}{\figWidth}};
\node at (-.7,1.6) {\small$\mu$};
\end{scope}
%
\begin{scope}[yshift=6cm]
\draw(-1.,0) node[anchor=south west] {\trimfig{Profile_eps7}{\figWidth}};
\draw(7.7,0) node[anchor=south west] {\trimfig{Profile_eps3}{\figWidth}};
\node at (-.7,1.6) {\small$\mu$};
\end{scope}
%
\begin{scope}[yshift=9cm]
\draw(-1.,0) node[anchor=south west] {\trimfig{Profile_eps8}{\figWidth}};
\draw(7.7,0) node[anchor=south west] {\trimfig{Profile_eps4}{\figWidth}};
\node at (-.7,1.6) {\small$\mu$};
\end{scope}
% background grid:
%\draw[step=1cm,gray] (0,0) grid (16,12.1);
\end{tikzpicture}
\end{center}
\caption{ Conservation of the adiabatic invariant~\eqref{eq: mu adiabatic} over 10000 iterations for the map generated by the symplectic gyroceptron~\eqref{eq: Composition NN Adiabatic Section} as $\varepsilon$ is increased.\label{fig: AdInv Profiles} }
\end{figure}
}

==> NPMap arXiv/plot.tex <==
{%you can use resizebox to rescale the picture
\def\layersep{2.5cm}
\begin{figure}[htb]
\begin{center}
\resizebox{20cm}{!}{% START resize box
\begin{tikzpicture}[    % GLOBAL CFG
    font=\sf \scriptsize,
    >=LaTeX,
    % Styles
    cell/.style={% For the main box
        rectangle, 
        rounded corners=5mm, 
        draw,
        very thick,
        },
    operator/.style={%For operators like +  and  x
        circle,
        draw,
        inner sep=-0.5pt,
        minimum height =.4cm,
        },
    function/.style={%For functions
        ellipse,
        draw,
        inner sep=1pt
        },
    ct/.style={% For external inputs and outputs
        circle,
        draw,
        line width = .75pt,
        minimum width=.9cm,
        inner sep=1pt,
        },
    gt/.style={% For internal inputs
        rectangle,
        draw,
        minimum width=4mm,
        minimum height=3mm,
        inner sep=1pt
        },
    mylabel/.style={% something new that I have learned
        font=\normalsize\sffamily
        },
    ArrowC1/.style={% Arrows with rounded corners
        rounded corners=.25cm,
        thick,
        },
    ArrowC2/.style={% Arrows with big rounded corners
        rounded corners=.5cm,
        thick,
        },]
\tikzstyle{backgroundblue}=[
    rectangle,
    fill=blue!10,
    inner sep=0.2cm,
    rounded corners=5mm
]
\tikzstyle{backgroundred}=[
    rectangle,
    fill=red!10,
    inner sep=0.2cm,
    rounded corners=5mm
]
\tikzstyle{backgroundgreen}=[
    rectangle,
    fill=green!10,
    inner sep=0.2cm,
    rounded corners=5mm
]

\useasboundingbox (0,0) rectangle (30,8); 
 
 %=================== HENON Layer ============================
\begin{scope}[xshift=12.8cm,yshift=6.5cm]
\node [backgroundgreen, minimum height =9.cm, minimum width=14.6cm] at (5.3,-2.7){} ;
 \node [] at (5.,1.5) {\Large H\'enonNet};
 \node [operator] (in1) at (-1.7,.5) {$q$};
 \node [operator] (in2) at (-1.7,-.5) {$p$};
 \node [cell, fill=green!40, minimum height =2.cm, minimum width=2.5cm] at (0,0){H\'enon Map} ;

 \node [operator] (in11) at (1.8,.5) {$q^{[1]}$};
 \node [operator] (in12) at (1.8,-.5) {$p^{[1]}$};

 \node [operator] (in21) at (5.3,.5) {$q^{[2]}$};
 \node [operator] (in22) at (5.3,-.5) {$p^{[2]}$};


 \node [operator] (in31) at (8.8,.5) {$q^{[3]}$};
 \node [operator] (in32) at (8.8,-.5) {$p^{[3]}$};
  \node [operator] (ou1) at (12.3,.5) {$\bar q$};
 \node [operator] (ou2) at (12.3,-.5) {$\bar p$};
 
  \draw [->, draw] (in1)-- (in11);
   \draw [->, draw] (in2)-- (in12);
     \draw [->, draw] (in11)-- (in21);
   \draw [->, draw] (in12)-- (in22);
        \draw [->, draw] (in21)-- (in31);
   \draw [->, draw] (in22)-- (in32);
           \draw [->, draw] (in31)-- (ou1);
   \draw [->, draw] (in32)-- (ou2);
   
\node [cell, fill=green!40, minimum height =2.cm, minimum width=2.5cm] at (0,0){H\'enon Map} ;
\node [cell, fill=green!40, minimum height =2.cm, minimum width=2.5cm] at (3.5,0){H\'enon Map} ;
\node [cell, fill=green!40, minimum height =2.cm, minimum width=2.5cm] at (7,0){H\'enon Map} ;
\node [cell, fill=green!40, minimum height =2.cm, minimum width=2.5cm] at (10.5,0){H\'enon Map} ;

\end{scope}
          
 %================ HENON NET =========================
\begin{scope}[xshift=17.8cm,yshift=2.4cm]
%Start drawing the thing...    
    % Draw the cell: 
    \node [cell, fill=green!40, minimum height =4.7cm, minimum width=6cm] at (0,-.5){} ;
     \node [rectangle, dashed, draw,  thick, minimum height =2.6cm, minimum width=3.4cm] at (-0.5,-1.5){} ;
    \node [] at (0.,2.2) {\Large H\'enon Map};
     \node [] at (-1.8,-2.6) {FNN};
    
    \node [ circle,draw, line width = .75pt, minimum width=.6cm,inner sep=1pt,fill=red!50] (ibox4) at (0.6,-1.5) {$V(p)$};

   % Draw opérators   named mux# , add# and func#
   % \node [operator] (mux1) at (-2,1.5) {$-I$};
    \node [operator] (nId) at (-0.5,1.5) {$-\cdot$};
    \node [operator] (mux2) at (-0.5,0.3) {$+\eta$};
    \node [operator] (mux3) at (2.4,-1.5) {$+$};
    \node [operator] (mux4) at (1.55,-1.5) {$\nabla$};
    %\node [function] (func1) at (1.5,0.75) {Tanh};
    
    \coordinate (x) at (-2.5,-0.75);
     \coordinate (y) at (1.5,1.5);
      \coordinate (z) at (2.7,.3);
       \coordinate (fnn) at (-1.8,-1.5);
       \node[] (cross) at (2.4,.3){};

    % Draw External inputs? named as basis c,h,x
    \node[ct, label={[mylabel]Input1}] (c) at (-4,1.5) {{\large$q$}};
    \node[ct, label={[mylabel]Input2}] (h) at (-4,-1.5) {{\large$p$}};
    
    %\node[ct, label={[mylabel]left:Input}] (x) at (-2.5,-3) {\empt{x}{t}};

    % Draw External outputs? named as basis c2,h2,x2
    \node[ct, label={[mylabel]Output1}] (c2) at (4,1.5) {\large$q^{[1]}$};
    \node[ct, label={[mylabel]Output2}] (h2) at (4,-1.5) {\large$p^{[1]}$};
   %Draw FNN
    \foreach \name / \y in {1,...,4}
        \node[circle, minimum size=12pt,inner sep=0pt, fill=blue!50] (I-\name) at (-.5, .15-\y/1.5) {};
     
    \foreach \name / \y in {1,...,4}
         \draw [->, thin, draw=black!50] (I-\name)--(ibox4);
         
      \foreach \name / \y in {1,...,4}
          \draw [->, thin, draw=black!50] (fnn)-- (I-\name);
% Start connecting all.
    %Intersections and displacements are used. 
    % Drawing arrows    
    \draw [ArrowC1] (c) -- (nId) -- (y);
    
      % Inputs
    \draw [thick] (h) --(fnn);
    \draw [ArrowC1] (h -| x)++(-0.5,0) -| (x);
    %\draw [ArrowC1] (h -| ibox3)++(-0.5,0) -| (ibox3);
    %\draw [ArrowC1] (x) -- (x |- h)-| (ibox3);

    % Internal
    \draw [-, ArrowC2] (x) |- (mux2);
    \draw [->, thick] (ibox4)--(mux4)-- (mux3);
    \draw [-, ArrowC1] (nId) -| (cross);
    \draw [->, thick] (cross)++(0.,-.15) -| (mux3);

    %Outputs
    \draw [->, thick] (mux3)++(0.2,0) |- (h2);
    \draw [->, ArrowC2] (mux2)++(0.2,0) --(z) |- (c2);
    \end{scope}
   

%%=================== INN Layer ============================
%\begin{scope}[xshift=10.7cm,yshift=6.5cm]
%\node [backgroundblue, minimum height =9.cm, minimum width=9.cm] at (1.7,-2.7){} ;
% \node [] at (2.,1.5) {\Large Coupling-based INN};
% \node [operator] (in1) at (-1.7,0) {$x$};
% \node [cell, fill=blue!40, minimum height =2.cm, minimum width=2.5cm] at (0,0){H\'enon Map} ;
% 
%\node [operator] (in11) at (1.8,0) {$x^{[1]}$};
%\node [operator] (ou1) at (5.3,0) {$\bar x$};
%
%\draw [->, draw] (in1)-- (in11);
%\draw [->, draw] (in11)-- (ou1);
%   
%\node [cell, fill=blue!40, minimum height =2.cm, minimum width=2.5cm] at (0,0){Coupling Flow} ;
%\node [cell, fill=blue!40, minimum height =2.cm, minimum width=2.5cm] at (3.5,0){Coupling Flow} ;
%
%\end{scope}
%
% %================ INN Map =========================
%\begin{scope}[xshift=12.4cm,yshift=2.4cm]
%%Start drawing the thing...    
%    % Draw the cell: 
%    \node [cell, fill=blue!40, minimum height =4.7cm, minimum width=6.5cm] at (0,-.5){} ;
%    \node [] at (0.,2.2) {\Large Coupling Flow};
%
%   % Draw opérators   named mux# , add# and func#
%   % \node [operator] (mux1) at (-2,1.5) {$-I$};
%    \node [operator] (plus) at (0.3,-2) {$+$};
%    \node [operator] (exp) at (-0.7,0.1) {$\exp(s(\cdot))$};
%    \node [operator] (t1) at (-.7,-2) {$t(\cdot)$};
%    \node [operator] (odot) at (-.7,-1.2) {$\odot$};
%    \node [operator] (linear) at (2.7,-.3) {$A\cdot + b$};
%    
%    \coordinate (x) at (-2.5,-0.75);
%     \coordinate (y) at (1.5,1.5);
%      \coordinate (z) at (2.7,.3);
%       \node[] (cross) at (2.4,.3){};
%
%    % Draw External inputs? named as basis c,h,x
%    \node[ct, label={[mylabel]Input}] (c) at (-4,-.3) {{\large$x$}};
%     \node[ct, label={[mylabel]Output}] (out) at (4,-.3) {{\large$x^{[1]}$}};
%    \node[gt] (k1) at (-2,1.) {{\large$x_{\le k}$}};
%     \node[gt] (k2) at (-2,-2) {\large{$x_{> k}$}};
%     
%     \node[gt] (o1) at (1.3,1.) {\large{$x_{\le k}$}};
%     \node[gt] (o2) at (1.3,-2) {\large{$\tilde x_{> k}$}};
%   \node[gt] (o3) at (1.8,-0.3) {\large{$\tilde x$}};
%    
%% Start connecting all.
%    %Intersections and displacements are used. 
%    % Drawing arrows    
%    \draw [ArrowC1] (c -| x)++(-1,0) -| (k1);
%     \draw [ArrowC1] (c -| x)++(-1,0) -| (k2);
%     \draw [ArrowC1] (k1 -| x)++(1,0) -| (exp) --(odot)--(plus);
%      \draw [->, thick] (k1) -- (o1);
%      \draw [->, thick] (plus) -- (o2);
%      
%     \draw [ArrowC1] (o3)++(-.2,0) -| (o1);
%     \draw [ArrowC1] (o3)++(-.2,0) -| (o2);
%    
%      % Inputs
%    \draw [thick] (k2) --(odot)--(plus);
%      \draw [thick] (k2) --(t1)--(plus);
%       \draw [->, thick] (o3) --(linear)--(out);
%
%    \end{scope}
    
    %=================== NN  ============================
\begin{scope}[xshift=1.4cm,yshift=6.5cm]
\node [backgroundred, minimum height =9.cm, minimum width=9.5cm] at (3.9,-2.7){} ;
  \node [] at (4,1.5) {\Large Symplectic Gyroceptron};
\node[ct, label={[mylabel]Input}] (c) at (0,-.5) {{\Large$(q, p)$}};
\node[ct, label={[mylabel]Output}] (o) at (6,-5) {{\Large$(\bar q, \bar p)$}};

\node[] (nn1p) at (3,-.8){};
\node[] (cross) at (1,-2){};
\node[] (center) at (6,-.5){};

 \node [cell, fill=red!40, minimum height =2.cm, minimum width=2.5cm] (nn1) at (3,-.5){\Large$\psi$} ;
  \node [cell, fill=red!40, minimum height =2.cm, minimum width=2.5cm] (nn2) at (3,-5){\Large$I_\epsilon$} ;
  \node [cell, fill=red!40, minimum height =2.cm, minimum width=3.5cm] (nn3) at (6.7,-.5){} ;
   \node [] at (8.,-1.2) {\Large$\Phi_\theta$};
   \node [] at (7.4,-.5) {\large$\theta$};
  
%now draw the circle
\draw[thick, ->] (center) arc (180:-155:.8);
\draw[dashed, ->] (6.4,-.5) arc (180:-155:.4);

    \draw [->, thick] (nn2)--(o);
     \draw [ArrowC1] (nn1p)++(-1.2,0) -| (cross);
      \draw [ArrowC1] (nn2)++(-1.2,0) -| (cross);
      \draw [->, thick] (1,-1)--(1,-3);
    \draw [->, thick] (c)--(nn1);
     \draw [->, thick] (nn1)--(nn3);
      \draw [->, thick] (5,-.8)--(4.2,-.8);
       \draw [->, thick] (6.1,-.8)--(5,-.8);
       \draw [->, thick] (5,-.5)--(6.05,-.5);
        \draw [dashed] (5,-.5)--(6.8,-.5);
        \draw [dashed] (6.1,-.8)--(6.8,-.5);
\end{scope}

 %grid:
% \draw[step=1cm,gray] (0,0) grid (30,8.);
 %
\end{tikzpicture}
}
\end{center}
\caption{Network diagrams. \  Left: Symplectic Gyroceptron. \  Right: H\'enon Network.
\label{fig:diagram}
\vspace{6mm} } 
\end{figure}
}


==> NPMap arXiv/trimFig.tex <==
% -------------------------------------------------------------------------------------
%
% Trim a figure: **NEW VERSION**
%  In this new version we hard code the original width of the plot to match an Overture figure.
%  The clipping parameters then denote fractions of this width (width=7.5 in = 19.05 cm)
%
%  \trimPlot{file}{width}{xa}{xb}{ya}{yb}
% Trim a figure and show the bounding box:
%  \trimPlotb{file}{width}{xa}{xb}{ya}{yb}
% 
%  file = name of the graphics file for includegraphics : .eps or pdf or ...
%  width : final width (after trimming) of the figure e.g. 5cm
%  xa,xb,ya,yb : trim this fraction of the width from the left, right, bottom and top
% 
% -----------------------------------------------------------------------------------------
\newlength{\tfwidth}
\newlength{\tfheight}
\newlength{\tfxa}
\newlength{\tfxb}
\newlength{\tfya}
\newlength{\tfyb}
% 
\newcommand{\trimPlotWithBox}[6]{%
\setlength\fboxsep{0pt}%
\setlength\fboxrule{1.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
}
\newcommand{\trimPlotNoBox}[6]{%
\setlength\fboxsep{1pt}% note: make this 1pt and rule thickness zero so box size matches that below
\setlength\fboxrule{0.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
% \includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}
}
% Trim a figure and draw the bounding box 
% Overture figures are 7.5 inches wide (8.5 - .5 -.5) = 19.05 cm
\newcommand{\trimPlotb}[6]{%
\setlength{\tfwidth}{19.05cm}%   % width of un-clipped fig
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfwidth*\real{#5}}%
\setlength{\tfyb}{\tfwidth*\real{#6}}%
% trim=l b r t
\trimPlotWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
% \trimPlotWithBox{#1}{#2}{#3}{#4}{#5}{#6}%
}
% Trim a figure 
% 
\newcommand{\trimPlot}[6]{%
\setlength{\tfwidth}{19.05cm}%   % width of un-clipped fig
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfwidth*\real{#5}}%
\setlength{\tfyb}{\tfwidth*\real{#6}}%
% trim=l b r t
\trimPlotNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}
% ----------------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------
%
% Trim a figure: 
%  \trimFig{file}{width}{xa}{xb}{ya}{yb}
% Trim a figure and show the bounding box:
%  \trimFigb{file}{width}{xa}{xb}{ya}{yb}
% 
%  file = name of the graphics file for includegraphics : .eps or pdf or ...
%  width : final width (after trimming) of the figure e.g. 5cm
%  xa,xb,ya,yb : trim this fraction of the width from the left, right, bottom and top
% 
% -----------------------------------------------------------------------------------------
\newcommand{\trimFigWithBox}[6]{%
\setlength\fboxsep{0pt}%
\setlength\fboxrule{1.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
}
% -----------------------------------------------------------------------------------------
\newcommand{\trimFigNoBox}[6]{%
\setlength\fboxsep{1pt}% note: make this 1pt and rule thickness zero so box size matches that below
\setlength\fboxrule{0.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
% \includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}
}
% ---------- Set height -----
\newcommand{\trimFigHeightWithBox}[6]{%
\setlength\fboxsep{0pt}%
\setlength\fboxrule{1.0pt}% border thickness
\fbox{\includegraphics[height=#2, clip, trim=#3 #4 #5 #6]{#1}}%
}
% ---------- Set height -----
\newcommand{\trimFigHeightNoBox}[6]{%
\setlength\fboxsep{1pt}% note: make this 1pt and rule thickness zero so box size matches that below
\setlength\fboxrule{0.0pt}% border thickness
\fbox{\includegraphics[height=#2, clip, trim=#3 #4 #5 #6]{#1}}%
% \includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}
}
% Trim a figure and draw the bounding box 
\newcommand{\trimFigb}[6]{%
\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
% trim=l b r t
\trimFigWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}
% Trim a figure 
% 
\newcommand{\trimFig}[6]{%
\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
% trim=l b r t
\trimFigNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

%%%%%%%%%%%%%% TRIMW : trim and set width %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% THIS VERSION WORKS PROPERLY %%%%%%%%%%%%%%%%%%
%  Thanks to Longfei Li
% New:
% Trim a figure (working) 
%  trims #3 #4 #5 #6 percent of left, right, bottom, top of the original figure
\newsavebox\figBox

\newcommand{\trimw}[6]{%
%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

% ----------------------------------------------------------------------------------------------
%%%%%%%%%%%%%% TRIMWB : trim and set width %%%%%%%%%%%%%%%%%%
%%%%%%%%%%   Version of trim that also draws the bounding box %%%%%%%%%%%%
\newcommand{\trimwb}[6]{%
%old: 
%\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
%\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
%new: Longfei 20160727: we should get the size of the original picture:
%\settowidth\tfwidth{\includegraphics{#1}}
%\settoheight\tfheight{\includegraphics{#1}}

%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

% ----------------------------------------------------------------------------------------------
%%%%%%%%%%%%%% TRIMH : trim and set height %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% THIS VERSION WORKS PROPERLY %%%%%%%%%%%%%%%%%%
%  Thanks to Longfei Li
% New:
% Trim a figure (working) 
%  trims #3 #4 #5 #6 percent of left, right, bottom, top of the original figure
\newcommand{\trimh}[6]{%
%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigHeightNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

% ----------------------------------------------------------------------------------------------
%%%%%%%%%%%%%% TRIMWB : trim and set height %%%%%%%%%%%%%%%%%%
%%%%%%%%%%   Version of trim that also draws the bounding box %%%%%%%%%%%%
\newcommand{\trimhb}[6]{%
%old: 
%\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
%\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
%new: Longfei 20160727: we should get the size of the original picture:
%\settowidth\tfwidth{\includegraphics{#1}}
%\settoheight\tfheight{\includegraphics{#1}}

%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigHeightWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}
% ----------------------------------------------------------------------------------------------
% 

